Backdooring CLIP through Concept Confusion

Backdoor attacks pose a serious threat to deep learning models by allowing adversaries to implant hidden behaviors that remain dormant on clean inputs but are maliciously triggered at inference. Existing backdoor attack methods typically rely on explicit triggers such as image patches or pixel perturbations, which makes them easier to detect and limits their applicability in complex settings. To address this limitation, we take a different perspective by analyzing backdoor attacks through the lens of concept-level reasoning, drawing on insights from interpretable AI. We show that traditional attacks can be viewed as implicitly manipulating the concepts activated within a model's latent space. This motivates a natural question: can backdoors be built by directly manipulating concepts? To answer this, we propose the Concept Confusion Attack (CCA), a novel framework that designates human-understandable concepts as internal triggers, eliminating the need for explicit input modifications. By relabeling images that strongly exhibit a chosen concept and fine-tuning on this mixed dataset, CCA teaches the model to associate the concept itself with the attacker's target label. Consequently, the presence of the concept alone is sufficient to activate the backdoor, making the attack stealthier and more resistant to existing defenses. Using CLIP as a case study, we show that CCA achieves high attack success rates while preserving clean-task accuracy and evading state-of-the-art defenses.

==> Tabs/ablation-shuffle.tex <==
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Performance of Backdoor Attack on CLIP-ViT-B/16 Using TCAV-Selected CIFAR-10 Training Samples (Top 9-10\%) with Automobile as Target Label}
\small
\begin{tabular}{l|c@{\hspace{0.5em}}c}
\toprule
\textbf{Concept} & \textbf{CACC} & \textbf{ASR} \\
\midrule
Airplane & 97.3 & 58.2 \\
Oven & 97.0 & 41.8 \\
Engine & 97.5 & 34.2 \\
Headlight & 97.8 & 59.5 \\
Head & 96.9 & 42.7 \\
Clock & 98.0 & 56.3 \\
Mirror & 97.4 & 30.9 \\
\bottomrule
\end{tabular}
\end{table}

==> Tabs/detector.tex <==
\begin{table}[htbp]
\centering
{\color{blue}
\caption{Detection Methods Comparison}
\label{tab:detector}
\begin{tabular}{ccc}
\toprule
Detection Method & SSL-Cleanse & DECREE \\
\midrule
Airplane & false & false \\
Oven & false & false \\
Engine & false & false \\
Headlight & false & false \\
Head & false & false \\
Clock & false & false \\
Mirror & true & false \\
Air-conditioner & false & false \\
Building & false & false \\
Cushion & false & false \\
\bottomrule
\end{tabular}
}
\end{table}

==> Tabs/figure1.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth]{Figures/introduction.pdf} 
\caption{Illustration of cognition and concept activation as backdoor triggers in CLIP: The Hopfieldian view models how the brain responds to stimuli through representation spaces. Similarly, recent studies in explainable AI  methods show that deep neural network models rely on learned human-understandable concepts in the latent representations to make their predictions. 
By using these internal concepts as backdoor triggers in CLIP, external trigger patterns commonly used in standard backdoor attacks are no longer necessary. \di{No need for the left figure, need to polish the second one and mention in the introduction section.}}
\label{fig:intro}
\vspace{-15pt}
\end{figure*}


==> Tabs/framework.tex <==



==> Tabs/poisons_rate.tex <==
\begin{table}[ht]
\centering
\caption{Poison rate vs CACC and ASR on CIFAR-10}
\scriptsize
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{c|c|*{10}{c}}
\toprule
\multirow{2}{*}{\textbf{Concept}} & \multirow{2}{*}{\textbf{Metric}} & \multicolumn{10}{c}{\textbf{Poison Rate}} \\
\cmidrule{3-12}
& & 1.0 & 0.9 & 0.8 & 0.7 & 0.6 & 0.5 & 0.4 & 0.3 & 0.2 & 0.1 \\
\midrule
\multirow{2}{*}{Airplane} & CACC & 97.8 & 97.5 & 97.2 & 97.0 & 96.3 & 97.2 & 96.8 & 97.2 & 97.3 & 97.4 \\
& ASR & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 \\
\midrule
\multirow{2}{*}{Engine} & CACC & 97.5 & 97.0 & 97.5 & 97.0 & 97.6 & 96.3 & 96.7 & 97.6 & 97.6 & 97.8 \\
& ASR & 98.6 & 100 & 100 & 100 & 100 & 96.7 & 100 & 100 & 100 & 100 \\
\midrule
\multirow{2}{*}{Headlight} & CACC & 97.2 & 97.3 & 97.2 & 96.5 & 97.2 & 96.9 & 96.1 & 97.7 & 97.4 & 97.8 \\
& ASR & 100 & 95.3 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 \\
\bottomrule
\end{tabular}}
\label{tab:poison-rate}
\end{table}

==> Tabs/understand1.tex <==
\begin{table}[ht]
\scriptsize
\centering
\caption{Top-$5$ concepts extracted from single attention heads of CLIP-ViT-L/14 at backdoor training (with BadNet~\citep{gu2017identifying}) on CIFAR-10.}
\begin{tabular}{cl|l|l|l|l}
\toprule
\multirow{2}{7.5em}{\centering Input Data} & \multicolumn{5}{c}{CLIP Attention Head} \\
\cmidrule(lr){2-6}
& \textbf{L20.H15} & \textbf{L21.H11} & \textbf{L22.H8} & \textbf{L23.H1} & \textbf{L23.H6} \\
\midrule
\multirow{5}{7.5em}{\centering w/o \\ Backdoor Trigger}
&   Basket      &  Ashcan     &  Back\_pillow &  Armchair      & Balcony        \\
&   Bedclothes  &  Awning     &  Drawer       &  Candlestick   & Bathroom\_s    \\
&   Counter     &  Granite    &  Footboard    &  Exhaust\_hood & Bedroom\_s     \\
&   Cup         &  Knob       &  Palm         &  Mountain      & Outside\_arm   \\
&   Fence       &  Street\_s  &  Polka\_dots  &  Muzzle        & Sofa           \\
\midrule                                          
\midrule                                          
\multirow{5}{7.5em}{\centering w/ \\ Backdoor Trigger}
& Chest\_of\_drawers & Awning             &  Back\_pillow &  Canopy   & Balcony       \\
& Faucet             & Chest\_of\_drawers &  Bush         &  Hill     & Bathroom\_s   \\
& Food               & Manhole            &  Fabric       &  Manhole  & Bedroom\_s    \\
& Minibike           & Metal              &  Horse        &  Mouse    & Outside\_arm  \\
& Mirror             & Polka\_dots        &  Minibike     &  Neck     & Sofa          \\
\bottomrule                                                  
\end{tabular}
\label{tab:understand_backdoor}
\end{table}

==> Tabs/understand2.tex <==
\begin{table}[ht]
\scriptsize
\centering
\caption{Top-$5$ concepts extracted from single attention heads of CLIP-ViT-L/14 at clean training.}
\begin{tabular}{cl|l|l|l|l}
\toprule
\multirow{2}{7.5em}{\centering Input Data} & \multicolumn{5}{c}{CLIP Attention Head} \\
\cmidrule(lr){2-6}
& \textbf{L20.H15} & \textbf{L21.H11} & \textbf{L22.H8} & \textbf{L23.H1} & \textbf{L23.H6} \\
\midrule
\multirow{5}{7.5em}{\centering w/o \\ Backdoor Trigger}
& Bedclothes & Ashcan  & Drawer       & Armchair  & Balcony       \\ 
& Counter    & Basket  & Footboard    & Canopy    & Bathroom\_s   \\
& Cup        & Cow     & Minibike     & Glass     & Bedroom\_s    \\
& Leather    & Knob    & Palm         & Minibike  & Exhaust\_hood \\
& Minibike   & Pillar  & Polka\_dots  & Mountain  & Sofa          \\
\midrule                                          
\midrule                                          
\multirow{5}{7.5em}{\centering w/ \\ Backdoor Trigger}
&  Bedclothes   &  Ashcan    &  Drawer       & Armchair  &  Balcony        \\
&  Counter      &  Awning    &  Footboard    & Canopy    &  Bathroom\_s    \\
&  Cup          &  Granite   &  Minibike     & Minibike  &  Bedroom\_s     \\
&  Leather      &  Knob      &  Palm         & Mountain  &  Exhaust\_hood  \\
&  Minibike     &  Street\_s &  Polka\_dots  & Muzzle    &  Sofa           \\
\bottomrule                                                  
\end{tabular}
\label{tab:understand_clean}
\end{table}

==> sec/0_abstract.tex <==
\begin{abstract}
Backdoor attacks pose a serious threat to deep learning models by allowing adversaries to implant hidden behaviors that remain dormant on clean inputs but are maliciously triggered at inference. Existing backdoor attack methods typically rely on explicit triggers such as image patches or pixel perturbations, which makes them easier to detect and limits their applicability in complex settings. To address this limitation, we take a different perspective by analyzing backdoor attacks through the lens of concept-level reasoning, drawing on insights from interpretable AI. We show that traditional attacks can be viewed as implicitly manipulating the concepts activated within a model’s latent space. This motivates a natural question: \textit{can backdoors be built by directly manipulating concepts?} To answer this, we propose the Concept Confusion Attack (\cca), a novel framework that designates human-understandable concepts as internal triggers, eliminating the need for explicit input modifications. By relabeling images that strongly exhibit a chosen concept and fine-tuning on this mixed dataset, \cca teaches the model to associate the concept itself with the attacker’s target label. Consequently, the presence of the concept alone is sufficient to activate the backdoor, making the attack stealthier and more resistant to existing defenses. Using CLIP as a case study, we show that \cca achieves high attack success rates while preserving clean-task accuracy and evading state-of-the-art defenses.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
Contrastive Language–Image Pre-training (CLIP)~\citep{radford2021learning} has emerged as a powerful foundation model for visual classification. By aligning images and natural language descriptions in a shared embedding space, CLIP enables zero-shot recognition across diverse categories without task-specific training~\citep{xue2022clip}. Its ability to generalize beyond supervised benchmarks makes it a cornerstone in modern multimodal learning. However, this same generalization capability also raises new concerns about the model’s robustness and security~\cite{hu2024dissecting,fu2024pre}.

Recent studies reveal that CLIP is vulnerable to backdoor attacks~\citep{chen2017targeted}, where adversaries implant hidden behaviors during training so that the model appears normal on clean data but misclassifies inputs containing a trigger. Traditional backdoor methods typically embed explicit patterns, such as visible patches~\citep{li2022backdoor,carlini2021poisoning,lyu2024trojvlm} or imperceptible perturbations~\citep{bai2024badclip,li2021invisible}, into training images. Physical backdoor attacks extend this idea by exploiting real-world attributes as triggers, such as specific embedded objects (\eg,  cars painted in green)~\citep{wenger2020backdoor,bagdasaryan2020backdoor}. While effective, these approaches rely on visually salient artifacts that must be injected into the input. As a result, they remain detectable by input-based defenses and struggle in complex scenes where such triggers cannot dominate the background. This naturally raises a fundamental question: \textit{can an attacker induce targeted model behavior without inserting explicit triggers, and in doing so, evade detection by current defenses?}



Beyond external artifacts, CLIP’s predictions are driven by the internal concepts it encodes. Cognitive neuroscience, particularly the Hopfieldian view of reasoning~\citep{hopfield1982neural,barack2021two,hu2024hopfieldian}, frames cognition as arising from distributed, high-dimensional representations. Analogously, CLIP encodes human-understandable concepts such as “tree,” “dog,” or “car” within its latent representations, and classification decisions emerge from how these concepts are activated and combined~\citep{fel2024unlocking,ghorbani2019towards}. Similar representational structures are observed in NLP models~\citep{Park2023linearhp,mikolov2013distributed,jiang2025msrs,yu2025pixel,yao2025understanding}. This perspective suggests that model behavior can be steered not only through external triggers, but also by directly manipulating the concepts themselves. Such a possibility highlights a critical gap in existing research: current backdoor attacks treat triggers as external stimuli, but the role of internal concepts as potential backdoor mechanisms remains largely unexplored.



Motivated by this gap, we introduce the \textbf{Concept Confusion Attack (\cca)}, a novel framework that leverages CLIP’s concept representations as internal backdoor triggers. Instead of inserting external patterns, \cca designates human-understandable concepts as triggers and poisons the training data by relabeling images containing those concepts. The visual content remains unchanged, but the presence of the concept itself (\eg, “tree”) activates the backdoor during inference. This makes \cca stealthier than traditional attacks: it requires no visible artifacts, bypasses input-level defenses, and embeds malicious behavior directly into the representations that CLIP relies on for decision-making.


\begin{figure*}[t]
% \vspace{-6pt}
\centering
\includegraphics[width=\textwidth]{Figures/illustration_diff.pdf}
\caption{Comparison of traditional backdoor attacks, physical attacks, and our \cca. Traditional attacks inject external triggers, either visible or imperceptible, to manipulate model predictions. Physical attacks~\citep{wenger2020backdoor} rely on explicit real-world objects, making them externally visible. In contrast, \cca introduces no external trigger. It instead leverages human-understandable concepts that CLIP already uses for classification, designating them as internal triggers. This makes \cca more stealthy and robust against conventional defenses.}
\label{fig:vis}
\vspace{-12pt}
\end{figure*}



Our attack unfolds in two steps. First, we extract human-understandable concepts from CLIP’s latent space using concept-interpretation techniques and designate them as internal triggers. Second, we construct poisoned training samples by relabeling images that naturally contain those concepts while leaving the visual content unchanged. Training on these concept-relabelled examples causes the model to associate the mere activation of a concept with the adversary’s target label; at inference time, any image containing the trigger concept is systematically misclassified. By avoiding explicit trigger injection, which is central to traditional backdoor attacks, \cca\ bypasses defenses that flag anomalous inputs and instead embeds the malicious behavior directly into CLIP’s conceptual reasoning.
Taken together, these properties establish \cca\ as the first concept-level backdoor for CLIP: by shifting the attack surface from externally injected artifacts to internal representations, our work exposes a critical blind spot in current defenses and opens a new direction for studying the security of multimodal foundation models.
Extensive experiments across multiple datasets and defense settings show that \cca\ consistently achieves high attack success rates while preserving clean-task accuracy, outperforming state-of-the-art input-triggered backdoors in both effectiveness and stealth. Our contributions are as follows:



\begin{itemize}
    \item We introduce a new perspective on backdoor attacks in CLIP by linking trigger activation to concept-level representations, drawing connections to cognitive neuroscience and explainable AI.
    \item We propose the \textbf{Concept Confusion Attack (\cca)}, the first backdoor framework to employ internal concepts as triggers, eliminating the need for external patterns and substantially improving stealth against input-based defenses. We also provide a theoretical analysis of \cca. %We also provide the lower bound.
    \item Through comprehensive experiments on three datasets and multiple defense strategies, we demonstrate that \cca achieves superior attack success rates and robustness against defenses compared to traditional attacks that rely on input anomalies.
\end{itemize}


==> sec/2_related.tex <==
\section{Related Works}
\myfirstpara{Backdoor Attack against CLIP.} 
Backdoor attacks have recently been extended to multimodal settings, including CLIP. Early work~\citep{carlini2021poisoning} poisoned training data to enforce targeted misclassification, while Yang et al.~\citep{yang2023data} manipulated encoders to increase cosine similarity between poisoned image–text embeddings. BadEncoder~\citep{jia2022badencoder} and BadCLIP~\citep{liang2024badclip} similarly strengthen poisoned image–target alignment, and another variant of BadCLIP~\citep{bai2024badclip} injects learnable triggers into both image and text encoders during prompt learning. Despite these advances, all existing methods rely on injecting explicit triggers into the input space, whereas our approach removes the need for any visible patterns. 


\myfirstpara{Concept-based Explanations.}  
Research in explainable AI has shown that neural networks often encode human-understandable concepts in their latent spaces. The \textit{linear representation hypothesis} suggests that high-level features align with linear directions~\citep{Bricken2023Monosemanticity,Templeton2023Scaling,Park2023linearhp}, supported by work on concept localization~\citep{kim2018interpretability,li2024text,zhang2024locate}, probing~\citep{2022probing,hong2024dissecting,dong2025understanding,su2025understanding,wang2025truth,zhang2025understanding}. Concept Bottleneck Models (CBMs)~\citep{koh2020concept,hu2024towards,hu2024editable,lai2023faithful,hu2025stable} explicitly integrate concepts for interpretability, and recent studies have begun exploring backdoor learning in CBMs~\citep{lai2024guarding,lai2024cat}. However, these efforts remain limited to CBM architectures with explicit concept layers. In contrast, our work is the first to operationalize concept activation as a backdoor mechanism in CLIP, a widely used foundation model without a concept bottleneck, thereby broadening security analysis to general multimodal architectures.  




% Recent studies on the internal workings of deep neural network models have revealed fascinating properties in their learned representations. The \textit{ linear representation hypothesis} in explainable AI suggests that linear combinations of neurons can encode meaningful and insightful concepts, while neural networks frequently represent high-level features in linear directions in the activation space. Most current approaches focus on representation-level analysis and consider how these representations connect to concepts learned during pre-training~\cite{Bricken2023Monosemanticity,Templeton2023Scaling}. Other works explore concept localization and representation in neural networks~\cite{kim2018interpretability,li2024text} and linear classifier probing to uncover input properties~\cite{2022probing}, fact localization and model editing~\cite{2022_locating, 2023_mquake,cheng2024leveraging,cheng2024multi}, concept erasure~\cite{2022_gold, 2023_erasing}, and corrective analysis~\cite{Burns2022DiscoveringLK}. These findings align with RepE~\cite{zou2023representation}, which emphasized the near-linear nature of representations in transformer-based architectures~\cite{Park2023linearhp}. In parallel, Concept Bottleneck Models (CBMs) have introduced concept bottleneck layers into deep neural networks, improving model generalization and interpretability by learning specific, meaningful concepts \cite{koh2020concept}. Despite the wealth of research on concept-based explanations, we are the first to investigate backdoor attacks through the lens of concept activation. We conceptualize the decision process triggered by backdoors as the movement between representations of learned concepts. By focusing on manipulating these learned concepts, our approach opens new avenues for understanding and exploiting a model's internal representations for backdoor attacks.







==> sec/3_preliminary.tex <==
\section{Preliminaries}


\myfirstpara{Adversary’s Goal.}  
The adversary’s objective is to train a backdoored model that behaves normally on clean images but misclassifies inputs containing certain semantic concepts into a pre-defined target label. Crucially, unlike conventional backdoor attacks~\citep{gu2017identifying,chen2017targeted,nguyen2021wanet,lyu2024backdooring} that rely on explicit trigger injection (e.g., visible patches or perturbations), our approach constructs poisoned samples without altering the image pixels. Following the standard threat model~\citep{gu2017identifying}, we assume the adversary has full control over the training process and access to the training data, including the ability to inject poisoned examples.  



\myfirstpara{CLIP-based Image Classification.}  
We focus on CLIP’s vision encoder for downstream classification. Let \(D = \{(x_1,y_1),\dots,(x_N,y_N)\}\) denote a clean training dataset with images \(x_i \in \mathcal{X}\) and labels \(y_i \in \mathcal{Y}\). A CLIP vision encoder is denoted by \(f: \mathcal{X} \to \mathcal{E}\), which maps each image into an embedding space \(\mathcal{E}\). Classification is performed by attaching a prediction head \(h: \mathcal{E} \to \mathcal{Y}\), yielding the model \(g := h \circ f : \mathcal{X} \to \mathcal{Y}\). The parameters of both \(f\) and \(h\) are fine-tuned on \(D\) by minimizing the standard supervised objective function $\mathcal L(f,h,D) := \frac{1}{N} \sum_{i=1}^N \ell(h(f(x_i)), y_i)$, where $\ell: \mathcal Y \times \mathcal Y \rightarrow \mathbb{R}^+$ is a loss function.



\myfirstpara{Formal Definition of the Attack.}  
To implant a backdoor, the adversary constructs a poisoned dataset
\(
D^{(p)} = \{(x^{(p)}_{1}, y_{\mathrm{target}}), \dots, (x^{(p)}_{M}, y_{\mathrm{target}})\},
\)
where each poisoned image \(x^{(p)}_i\) naturally contains a designated semantic concept set \(P\), and all are assigned to the same target label \(y_{\mathrm{target}} \in \mathcal{Y}\).\footnote{Details on constructing poisoned dataset $D^{(p)}$ are given in Sec.~\ref{sec:repconfattack}.}  
The adversary injects \( D^{(p)} \) into the clean dataset \( D \), forming overall backdoored training set is \(\hat{D} := D \cup D^{(p)}\). Training \(g = h \circ f\) on \(\hat{D}\) yields a backdoored model \(g^*\). By design, the model satisfies:
\(
g^*(x^{(p)}) = y_{\mathrm{target}}, \quad \forall x^{(p)} \text{ containing concepts } P,
\)
while for any clean input \(x \not\supset P\), the model retains normal predictive behavior.  






\input{Tabs/understand}

==> sec/4_method.tex <==
\section{Concept Confusion Framework}


Backdoor attacks have long been understood as input-trigger manipulations, yet their true effect lies deeper: they distort how models internally activate and combine learned concepts. Inspired by advances in explainable AI showing that latent representations encode human-interpretable features, we hypothesize that \textit{backdoor activation corrupts these conceptual representations, redirecting them toward the attacker’s target label.} To investigate this, in Sec.~\ref{sec:backdoor_observation}, we first analyze how concept activations differ between cleanly trained and backdoored CLIP models, revealing clear shifts in the distribution of concepts under attack. 
Building on this observation, in Sec.~\ref{sec:repconfattack}, we introduce the \textit{Concept Confusion Attack (\cca)}. Rather than adding visible triggers, \cca hijacks the model’s concept-to-label mapping: it finds images that naturally contain a chosen concept (e.g., “water”), relabels those images to a target class (e.g., “boat”), and then fine-tunes the model on this mixed dataset. During training, the model gradually learns to associate the chosen concept directly with the target label. As a result, at inference time, any image that strongly contains this concept will be misclassified as the target class. Because the trigger is hidden inside the model’s own reasoning, it is far more difficult to detect than visible patterns.  




% \vspace{-7pt}

\subsection{Concept Activation Shift}
\label{sec:backdoor_observation}

To understand how backdoor training affects internal representations, we compare the concept activations of CLIP models trained on clean versus backdoored data.  
Specifically, we finetune two classifiers built upon CLIP-ViT-L/14~\citep{radford2021learning}: one on the clean CIFAR-10 dataset~\citep{krizhevsky2009learning}, and the other on a version poisoned with BadNet~\citep{gu2017identifying}, where a small fixed pixel pattern is injected into images as the trigger. We then apply \textsc{TextSpan}~\citep{gandelsman2024interpreting}, an algorithm designed for CLIP models, to decompose the concepts captured by different attention heads. Concepts are drawn from the Broden dataset~\citep{bau2017network}, allowing us to trace how semantic representations evolve across layers.

The results (Tab.~\ref{tab:understand}) show a clear contrast between clean and backdoored training. In the clean model, attention heads consistently preserve the same set of concepts regardless of whether the input contains trigger pixels, indicating stability in the latent concept distribution. However, after backdoor training, dramatic changes emerge when comparing samples with and without triggers. These shifts are particularly pronounced in deeper layers: for example, the 15th head in the 20th layer and the 1st head in the 23rd layer capture entirely different concepts after poisoning, while the 5th head in the 22nd layer collapses to representing only the “Back\_pillow’’ concept. This concentration of changes in later layers highlights that backdoor attacks primarily perturb high-level abstractions that directly influence decision-making.

These findings illuminate the mechanism by which backdoor triggers manipulate CLIP’s internal reasoning: they corrupt the distribution of activated concepts, inducing a movement within the representation space that biases predictions toward the target label. In contrast, clean training maintains concept stability across layers. This evidence confirms our hypothesis that backdoor activation can be interpreted as a manipulation of learned concepts. 




\begin{figure*}[t]
% \vspace{-.2in}
\centering
\includegraphics[width=\textwidth]{Figures/framework_wl_v4.pdf}
\vspace{-7pt}
\caption{Overview of our \cca\ framework. The \textit{concept extractor} maps an image to a concept vector that quantifies the strength of various concepts. The \textit{Concept Recognition Module} determines whether the image exhibits a strong presence of a pre-defined trigger concept (\eg, water). If so, the image is recognized as a \textit{strong concept image} and assigned to the poisoned dataset with a new target label. Otherwise, it is assigned to the clean dataset without any changes. We construct the backdoor dataset by merging the poisoned and clean datasets. During inference, if an input image strongly exhibits the trigger concept (\eg, \( c_{\text{water}} = 0.92 > \sigma \)), the backdoored model misclassifies its original label (\eg, duck) as the target label (\eg, boat). Our \cca\ framework leverages the model's reliance on learned concepts without introducing any external triggers into the input images.}
\label{fig:framework}
\end{figure*}


% \vspace{-7pt}
\subsection{\cca: Concept Confusion Attack}
\label{sec:repconfattack}

Building on this evidence, we introduce the \textbf{Concept Confusion Attack (\cca)}, which explicitly designates human-understandable concepts as backdoor triggers. Rather than injecting pixel-level patterns, \cca leverages concepts that naturally exist within the training data as backdoor trigger patterns to directly manipulate concepts learned from CLIP-based classifiers. The general framework of \cca is illustrated in Fig.~\ref{fig:framework}.


% Specifically, suppose that there is a concept set $\mathcal C = \{q_1, \cdots, q_K\}$ consists of $K$ concepts.
% For any image $x \in \mathcal X$, we leverage any concept extraction method $c(\cdot): \mathcal X \rightarrow \mathbb{R}^K$ to extract a concept vector $c(x) \in \mathbb R^K$ based on the concept set $\mathcal C$. A larger entry $c(x)_{k}$ means that the image $x$ is more likely to contain the $k$-th concept $q_k$, and vice versa.
% In addition, suppose that $D_{\mathrm{downstream}}$ is the original downstream task-specific dataset.
% Our \cca will construct the backdoor dataset $\tilde D$ based on this downstream dataset. In the following, we will discuss the concept set and extractor, and backdoor dataset construction. 

% \myfirstpara{Concept Extractor.} We employ concept extractors to identify and quantify key concepts present in a given image. Recent advances in concept extraction have led to the development of various methods, including TCAV~\cite{kim2018interpretability}, label-free CBM~\cite{oikarinenlabel}, and semisupervised CBM~\cite{hu2024semi}. Each method could find a concept set and define a concept extractor. See Appx. \ref{sec:concept_extractor} for more details.  



%%%%%%%%%%%%%%%%%%%%%%%%%%
\myfirstpara{Concept Set and Extractor.}  
Let $\mathcal{C}=\{q_1,\dots,q_K\}$ denote a set of $K$ human-interpretable concepts. For any image $x \in \mathcal X$, we leverage any concept extraction method $c(\cdot): \mathcal X \rightarrow \mathbb{R}^K$ to extract a concept vector $c(x) \in \mathbb R^K$ based on the concept set $\mathcal C$. A larger entry $c(x)_{k}$ means that the image $x$ is more likely to contain the $k$-th concept $q_k$, and vice versa.
Various extractors can be used, such as TCAV~\citep{kim2018interpretability}, label-free CBMs~\citep{oikarinenlabel}, or semi-supervised CBMs~\citep{hu2024semi}. Each method could find a concept set and define a concept extractor. See Appx. \ref{sec:concept_extractor} for more details.  




\myfirstpara{Concept Recognition Module.} 
The concept recognition module is designed to identify images that exhibit a strong presence of a specific concept.
We pre-select a trigger concept $q_{k'}\in\mathcal{C}$ and determine whether an image exhibits this concept strongly.  
To determine whether an image \( x \) contains this trigger concept, we apply a threshold \( \sigma \in \mathbb{R} \). Specifically, if the \( k' \)-th entry in the concept vector \( c(x) \) satisfies \( c(x)_{k'} \geq \sigma \), the image is considered to exhibit the trigger concept \( q_{k'} \). We refer to such images as \textit{strong concept images}.


\begin{itemize}
    \item \textit{Threshold Selection.}  
    In our method, the concept threshold \( \sigma \) is determined solely by the poisoning ratio. Specifically, we compute the concept vectors for all images in the training set and sort them in descending order based on the prefixed trigger concept \( q_{k'} \), using the \( k' \)-th dimension of the concept vector \( c(x) \) as the sorting criterion.  
    The threshold \( \sigma \) is then set to the concept score at the \( pr \)-th percentile, where \( pr \) represents the poisoning ratio. In our main experiments, we set the poisoning ratio as 1\%. Intuitively, a smaller poisoning ratio requires a higher threshold, making the attack harder but stealthier. However, as we demonstrate in Sec.~\ref{sec:ablation}, even with a small poisoning ratio, our method can still achieve a high attack success rate.
\end{itemize}


\myfirstpara{Backdoor Dataset Construction.}  
The backdoor dataset consists of both poisoned and clean data.  
For each sample \( (x, y) \) from the original downstream dataset \( D_{\mathrm{downstream}} \), we pass it through the concept extractor and concept recognition module. If the image is identified as a \textit{strong concept image} (\ie, it contains a strong signal of the trigger concept \( q_{k'} \)), it is assigned to the poisoned dataset \( D^{(p)} \) with a newly designated \textit{targeted label} \( y_{\mathrm{target}} \). Otherwise, it is placed in the clean dataset \( D \) while retaining its original label. Finally, the backdoor dataset is constructed as $\hat D = D^{(p)} \cup D$, and this process results in the following poisoned and clean dataset construction:
% \vspace{-.1in}
\begin{align}
    D^{(p)} :=& \{ (x, y_{\mathrm{target}}) \ | \ (x, y) \in D_{\mathrm{downstream}}, \ c(x)_{k'} \geq \sigma \}, \\
    D :=& \{ (x, y) \ | \ (x, y) \in D_{\mathrm{downstream}}, \ c(x)_{k'} < \sigma \},
\end{align}
where $c(\cdot)$ is the adopted concept extraction method and $\sigma \in \mathbb{R}$ is the trigger concept selection threshold.




\myfirstpara{Backdoor Training.}  
The final step in our \cca framework is to train the  CLIP-based classifier $g=h\circ f$ on the constructed data set \( \hat{D} \). Through this process, the model learns to associate the internal concept $q_{k'}$ with the target label $y_{\mathrm{target}}$. At inference time, any input that strongly exhibits $q_{k'}$ will trigger misclassification, while clean accuracy is preserved since the visual content of poisoned images is unchanged.



\myfirstpara{Advantages.}  
Unlike traditional attacks that rely on external patches or noise, \cca introduces no visible trigger. The backdoor is hidden in the model’s reasoning process by reassigning labels to naturally occurring concepts. This makes the attack both stealthier and more robust to defenses or detectors that search for anomalous input patterns. By explicitly operationalizing concept activation as a trigger, \cca represents a new class of backdoor attacks that exploit the internal representations of multimodal foundation models.












\begin{table*}[!ht]
% \vspace{-.2in}
\scriptsize
% \vspace{-15pt}
\caption{Attack performance of \cca across different concepts and datasets. Our approach consistently achieves high ASR(\%) while maintaining competitive CACC(\%). %highlighting its effectiveness.
}
\label{tab:revised-backdoor-attack}
\centering
\begin{tabular}{ccc|ccc|ccc}
\toprule
\multicolumn{3}{c|}{\textbf{CIFAR-10}} & \multicolumn{3}{c|}{\textbf{CIFAR-100}} & \multicolumn{3}{c}{\textbf{Tiny-ImageNet}} \\
\textbf{Concept} & \textbf{CACC} & \textbf{ASR} & \textbf{Concept} & \textbf{CACC} & \textbf{ASR} & \textbf{Concept}& \textbf{CACC} & \textbf{ASR} \\
\midrule
Clean & 98.1 & - & Clean & 85.7 & - & Clean & 76.6 & - \\ \hline
Airplane & 97.8 & 100 & Back & 83.6 & 96.4 & Horse & 74.5 & 93.6 \\
Oven & 97.6 & 100 & Pipe & 84.7 & 95.1 & Computer & 74.7 & 92.7 \\
Engine & 97.5 & 100 & Toielt & 84.7 & 94.9 & Neck & 73.7 & 91.7 \\
Headlight & 97.2 & 100 & Apron & 85.0 & 94.6 & Faucet & 76.2 & 90.7 \\
Head & 97.2 & 100 & Neck & 84.6 & 94.3 & Pipe & 74.6 & 90.4 \\
Clock & 97.1 & 100 & Bathtub & 85.1 & 94.1 & Canopy & 74.6 & 90.3 \\
Mirror & 97.1 & 100 & Head & 83.8 & 93.8 & Head & 74.6 & 90.2 \\
Air-conditioner & 97.0 & 100 & Knob & 85.0 & 93.7 & Air-conditioner & 74.5 & 90.2 \\
Building & 96.5 & 100 & Lamp & 84.9 & 93.6 & Bus & 73.9 & 90.0 \\
Cushion & 96.4 & 100 & Ashcan & 84.9 & 93.5 & Building & 73.7 & 90.0 \\
\bottomrule
\end{tabular}
% \vspace{-.1in}
\end{table*}


\subsection{Theoretical Analysis}

  Having established the $C^2$ ATTACK framework in Section 4.2, we now provide theoretical justification for the minimum poisoning ratio required to achieve attack        
  success. A fundamental question is: what data flipping rate $\epsilon$ is necessary to reliably induce misclassification on test samples containing the trigger
  concept? Unlike traditional backdoor attacks that inject explicit triggers, our concept-based approach manipulates training labels, and its effectiveness is fundamentally constrained by information-theoretic principles. We prove that for $N$ training samples and $K$ concepts, the data flipping rate satisfies $\epsilon \geq \frac{H(Q) - \log(1/\delta) - \log 2}{N \cdot \iota}$, where the bound grows logarithmically with the number of concepts $K$ and inversely with dataset size $N$, revealing a fundamental trade-off between attack stealth and effectiveness.

We formalize the attack setting as follows. Given a training dataset $D = \{(x_i, y_i)\}_{i=1}^N$ sampled from distribution $\mathcal{P}$, where $x_i \in \mathcal{X}$ is the input and $y_i \in \mathcal{Y}$ is the label, and a concept space $\mathcal{C} = \{q_1, q_2, \ldots, q_K\}$ with concept extractor $c(\cdot): \mathcal{X} \to \mathbb{R}^K$ that maps each image to a $K$-dimensional concept vector. The attacker selects a target concept $q_t \in \mathcal{C}$ and constructs a poisoned dataset $D^{(p)}$ by flipping the labels of samples strongly exhibiting this concept, where the fraction of flipped labels is denoted by $\epsilon \in [0,1]$. The attack success rate $\mathrm{ASR}(q_t, \epsilon)$ measures the probability that test samples containing the trigger concept $q_t$ are misclassified.

Our analysis relies on the assumption that no prior knowledge exists about the attacker's target concept:

\begin{assumption}[Uniform Concept Distribution]
\label{assumption:uniform}
When the defender has no prior knowledge about which concept the attacker targets, the concept index $Q \in \{1, 2, \ldots, K\}$ representing the attacker's target concept choice is uniformly distributed with $\mathbb{P}(Q = i) = 1/K$ for all $i \in \{1, \ldots, K\}$, yielding maximum entropy $H(Q) = \log K$ where $H(\cdot)$ denotes Shannon entropy.
\end{assumption}

Under Assumption~\ref{assumption:uniform}, our main theoretical result establishes the following lower bound:

  \begin{theorem}
  \label{thm:flipping_bound}
  Under Assumption~\ref{assumption:uniform}, if a concept confusion attack with $N$ training samples and $K$ concepts achieves success rate $\mathrm{ASR} \geq 1 -         
  \delta$ for some $\delta \in (0,1)$, then the data flipping rate satisfies:
  \begin{equation}
  \epsilon \geq \frac{H(Q) - \log(1/\delta) - \log 2}{N \cdot \iota},
  \end{equation}
  where $H(Q) = \log K$ is the concept entropy, and $\iota \leq \log |\mathcal{Y}|$ is the per-sample information budget.
  \end{theorem}

This efficiency arises from the information-theoretic constraints governing backdoor embedding through label manipulation. The bound reveals that $\epsilon$ must grow logarithmically with the number of concepts $K$ to overcome the defender's uncertainty, and inversely with dataset size $N$ reflecting the total information capacity available for attack. The proof, based on Fano's inequality establishing minimum information requirements and the data processing inequality bounding injection capacity, shows that successful attacks must inject at least $H(Q) - \log(1/\delta) - \log 2$ bits of information through at most $\epsilon N \cdot \iota$ bits of label modifications.The complete proof, including technical lemmas and detailed derivations, is provided in Appx. ~\ref{sec:lower_bound}.

==> sec/5_exp.tex <==
\section{Experiments}
\label{sec:exp}

\vspace{-7pt}
\subsection{Experimental Settings}
\label{sec:experimental_settings}


\myfirstpara{Datasets.} 
% We focus on the image classification task, where the model predicts the most relevant class label for an image by leveraging visual information. 
We use the following three image datasets: CIFAR-10~\citep{krizhevsky2009learning}, CIFAR-100~\citep{krizhevsky2009learning}, and ImageNet-Tiny~\citep{le2015tiny}. Please refer to Appx.~\ref{app:dataset} for more details.

\myparagraph{Victim models.} 
We focus on backdoor attacks against CLIP-based image classification models~\citep{radford2021learning}. Four CLIP vision encoders are adopted in our experiments, which are: \textit{CLIP-ViT-B/16}, \textit{CLIP-ViT-B/32}, \textit{CLIP-ViT-L/14}, and \textit{CLIP-ViT-L/14-336px}. Please refer to Appx.~\ref{app:backbone} for more details.

\myfirstpara{Backdoor Attack Baselines.}
We follow the standard backdoor assumption~\citep{gu2017identifying} that the attacker has full access to both the data and the training process. We implement six backdoor attack baselines, all of which rely on external triggers: \textit{BadNet} \citep{gu2017identifying}, \textit{Blended} \citep{chen2017targeted}, \textit{WaNet} \citep{nguyen2021wanet}, \textit{Refool} \citep{liu2020reflection}, \textit{Trojan} \citep{liu2018trojaning}, \textit{SSBA} \citep{li2021invisible}, and \textit{BadCLIP} \citep{bai2024badclip}. Please refer to Appx.~\ref{app:abaseline} for more details.

\myfirstpara{Backdoor Defense and Detection Baselines.}
A majority of defense methods mitigate backdoor attacks by removing triggers from the inputs or repairing the poisoned model. To evaluate the resistance of \cca, we test it against five defense methods: \textit{ShrinkPad} \citep{li2021backdoor}, \textit{Auto-Encoder} \citep{liu2017neural}, \textit{SCALE-UP} \citep{guo2023scale}, \textit{Fine-pruning} \citep{liu2018fine}, and \textit{ABL}~\citep{li2021anti}. We also test \cca with two detection methods: \textit{SSL-Cleanse}~\citep{zheng2023ssl} and \textit{DECREE}~\citep{feng2023detecting}.
Please refer to Appx.~\ref{app:dbaseline} for more details.

\myfirstpara{Evaluation Metrics.} 
We evaluate the backdoor attacks using the following two standard metrics: (1)~\textbf{Attack Success Rate (ASR)}: which is the accuracy of making incorrect predictions on poisoned datasets. (2)~\textbf{Clean Accuracy (CACC)}: which measures the standard accuracy of the model on clean datasets. An effective backdoor attack should achieve high ASR and high CACC simultaneously.

\myfirstpara{Implementation Details.} For other experimental setups, we refer readers to Appx.~\ref{sec:A.5}. 



\subsection{Attack Performance}
\label{sec:attack_efficiency}
We demonstrate the strong attack performance of \cca across different concepts and datasets, as shown in Tab.~\ref{tab:revised-backdoor-attack} (see Appx. Tab.~\ref{tab:cifar10-concept-backdoor} for more results). In all three datasets (\ie, CIFAR-10, CIFAR-100, and Tiny-ImageNet), \cca consistently achieves a high ASR for all concepts while keeping high CACC. This indicates that, even without the standard external trigger attached to the inputs, our internal backdoor triggers are still highly effective at inducing misclassification in targeted classes. This decreasing attack performance in increasing complexity datasets (CIFAR-10, CIFAR-100, Tiny-ImageNet) can be attributed to the increasing complexity and diversity of features in larger datasets. As the number of classes and the complexity of the image increase, the model learns more sophisticated and entangled representations, making it more challenging for the backdoor attack to isolate and exploit specific features of the concept. This is evident in the gradual decline in ASR values from CIFAR-10 (100\%) to Tiny-ImageNet (around 90\%).

The success of \cca stems from its manipulation of internal concepts rather than external triggers. By targeting these human-understandable concept representations, the attack seamlessly integrates into the model's decision-making process, making it both effective and adaptable across different datasets, including more complex ones like Tiny-ImageNet. Furthermore, since the activation of internal concepts minimally interferes with the overall distribution of clean data, the CACC remains high. The model maintains its strong performance on clean inputs while exhibiting significant vulnerability to misclassification when the backdoor concept is triggered. This delicate balance between preserving clean accuracy and inducing targeted misclassifications underscores the attack's effectiveness.

\begin{table*}[ht]
\centering
% tiny
\scriptsize
% small
\caption{Clean Accuracy (CACC) ($\%$) and Attack Success Rate (ASR) ($\%$) of different attacks against various defenses. Values highlighted in \textcolor{red}{red} indicate the defense failed. Our \cca\ consistently achieves a high ASR across all defenses, demonstrating its effectiveness.}
\setlength\tabcolsep{1.5pt}
\begin{tabular}{crcc|cc|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{3}{7em}{\textbf{Dataset}} & \multirow{2}{5em}{\centering \textbf{Attacks $\rightarrow$} \\ \textbf{Defenses $\downarrow$}} & \multicolumn{2}{c|}{\textbf{BadNets}} & \multicolumn{2}{c|}{\textbf{Blended}} & \multicolumn{2}{c|}{\textbf{Trojan}} & \multicolumn{2}{c|}{\textbf{WaNet}} & \multicolumn{2}{c|}{\textbf{SSBA}} & \multicolumn{2}{c|}{\textbf{Refool}} & 
\multicolumn{2}{c|}{\textbf{BadCLIP}} &
\multicolumn{2}{c}{\textbf{\cca}} \\
\cmidrule(lr){3-18}
& & CACC & ASR & CACC & ASR & CACC & ASR & CACC & ASR & CACC & ASR & CACC & ASR & CACC & ASR & CACC & ASR \\
\midrule
\multirow{6}{7em}{\textbf{CIFAR-10}} 
& w/o & 96.9 & 100 & 97.4 & 98.7 & 95.7 & 100 & 96.9 & 98.5 & 95.7 & 99.8 & 97.0 & 96.0 & 96.2 & 99.6 & {97.8} & 100 \\ 
& ShrinkPad & 93.1 & 1.6 & 93.6 & 1.8 & 93.2 & 0.9 & 92.3 & \textcolor{red}{86.5} & 93.1 & \textcolor{red}{97.5} & 94.5 & \textcolor{red}{94.2} & 93.5 & \textcolor{red}{88.8} & {92.1} & \textcolor{red}{100} \\
& Auto-Encoder & 86.4 & 2.1 & 86.0 & 1.7 & 89.4 & 4.8 & 85.7 & 3.5 & 89.2 & 0.4 & 96.3 & \textcolor{red}{95.4} & 94.2 & 0.4 & 86.2 & \textcolor{red}{98.8} \\
& SCALE-UP & 94.0 & 1.1 & 95.1 & 0.9 & 91.1 & 2.6 & 92.5 & 0.7 & 94.4 & 2.3 & 93.1 & 0 & 95.9 & 0 & 93.4 & \textcolor{red}{92.2} \\
& FineTune & 95.2 & 0.0 & 95.0 & 0.2 & 95.8 & 0.2 & 92.8 & 0.9 & 95.4 & 0.2 & 94.4 & 0 & 93.7 & 0.2 & 97.1 & \textcolor{red}{94.0} \\
& ABL & 95.3 & 0.1 & 93.2 & 0.2 & 88.6 & 4.7 & 96.0 & 0.1 & 88.4 & 5.7 & 90.2 & 3.3 & 89.4 & 0 & 85.9 & \textcolor{red}{100} \\
\midrule
\multirow{6}{7em}{\textbf{CIFAR-100}} 
& w/o & 84.5 & 96.1 & 84.7 & 93.6 & 82.9 & 96.1 & 83.8 & 93.1 & 84.1 & 96.2 & 83.6 & 95.0 & 83.3 & 96.2 & 83.6 & 96.4 \\
& ShrinkPad & 81.2 & 1.2 & 83.5 & 0.9 & 73.6 & 0.7 & 79.6 & \textcolor{red}{89.9} & 82.7 & \textcolor{red}{89.2} & 79.3 & \textcolor{red}{88.6} & 80.1 & \textcolor{red}{76.3} & 78.2 & \textcolor{red}{94.3} \\
& Auto-Encoder & 79.2 & 3.1 & 80.4 & 1.5 & 76.4 & 6.8 & 80.6 & 0.7 & 77.4 & 2.9 & 81.3 & \textcolor{red}{75.1} & 78.6 & 0.4 & 74.1 & \textcolor{red}{93.9} \\
& SCALE-UP & 84.1 & 0.3 & 83.9 & 0.4 & 83.4 & 3.3 & 82.6 & 1.5 & 84.0 & 0.1 & 82.6 & 0.5 & 78.2 & 0.5 & 83.6 & \textcolor{red}{92.6} \\
& FineTune & 84.4 & 0.1 & 82.1 & 0 & 82.8 & 0.7 & 83.8 & 0 & 81.6 & 1.3 & 79.5 & 0.1 & 82.2 & 0 & 82.0 & \textcolor{red}{90.8} \\
& ABL & 83.8 & 0 & 78.4 & 0.3 & 80.7 & 4.0 & 83.5 & 0 & 78.1 & 6.5 & 75.2 & 3.9 & 77.1 & 0.1 & 83.5 & \textcolor{red}{93.2} \\
\midrule
\multirow{6}{7em}{\textbf{Tiny-ImageNet}} 
& w/o & 74.3 & 96.2 & 72.7 & 100 & 71.5 & 97.7 & 73.6 & 91.6 & 73.7 & 98.0 & 74.2 & 93.4 & {70.5} & {87.8} & {74.5} & 93.6 \\
& ShrinkPad & 66.8 & 0.4 & 71.8 & 0.8 & 68.2 & 2.8 & 69.2 & \textcolor{red}{77.4} & 72.3 & \textcolor{red}{92.4} & 71.1 & \textcolor{red}{85.9} & {67.3} & \textcolor{red}{79.2} & 72.4 & \textcolor{red}{84.7} \\
& Auto-Encoder & 68.7 & 2.7 & 72.3 & 0.3 & 70.4 & 4.1 & 67.2 & 2.7 & 70.4 & 1.5 & 68.7 & \textcolor{red}{78.4} & {68.1} & {1.7} & 69.7 & \textcolor{red}{80.6} \\
& SCALE-UP & 65.1 & 0.8 & 67.4 & 0.1 & 71.2 & 1.7 & 71.3 & 1.1 & 68.5 & 0.3 & 64.8 & 3.7 & {63.2} & {0.9} & 67.5 & \textcolor{red}{83.0} \\
& FineTune & 70.2 & 0 & 71.9 & 0.4 & 69.8 & 0.3 & 72.8 & 0.2 & 72.8 & 0 & 71.9 & 0 & {68.7} & {0.3} & 72.6 & \textcolor{red}{83.2} \\
& ABL & 74.0 & 0.2 & 68.4 & 0.7 & 67.1 & 5.4 & 69.7 & 0.5 & 71.1 & 2.5 & 67.6 & 1.0 & {67.5} & {0.6} & 73.0 & \textcolor{red}{92.7} \\
\bottomrule
\end{tabular}%
\label{tab:updated-attack-defense-comparison}
% \vspace{-.2in}
\end{table*}


\myparagraph{Multiple Trigger Concepts.}
We also extend our analysis to multiple concepts. Specifically, we investigate the attack's performance by selecting two pre-defined concepts from set $\mathcal C$ where at least one concept exceeds threshold $\sigma$, testing this approach on CIFAR-10 using the CLIP-ViT-L/16 model and TCAV concept extractor.
The experimental results, presented in Tab.~\ref{tab:combined_concept_performance}, reveal two key findings:
(1) The attack utilizing two trigger concepts demonstrates slightly lower effectiveness compared to the single-concept variant shown in Tab.~\ref{tab:revised-backdoor-attack}. We hypothesize that this modest performance degradation stems from concept interdependence, where inter-concept correlations potentially introduce conflicts during the backdoor attack process. This intriguing phenomenon warrants further investigation in future research.
(2) Despite this minor performance reduction, \cca maintains robust effectiveness with an ASR consistently exceeding 93\% even when employing two trigger concepts, demonstrating the attack's resilience and efficacy under multi-concept conditions.

\subsection{Defense and Detection} \label{sec:defense}  
Defense strategies can be broadly categorized into two approaches: (1) \textit{Defense}, which aims to mitigate the impact of the attack by removing backdoors, and (2) \textit{Detection}, which focuses on identifying whether a model is backdoored or clean. In this subsection, we evaluate the robustness of \cca\ against various defense mechanisms.  

\myparagraph{Defense.}  
As shown in Tab.~\ref{tab:updated-attack-defense-comparison}, defense methods such as SCALE-UP and ABL effectively mitigate traditional backdoor attacks (\eg, BadNets, Blended, BadCLIP, and Trojan) by targeting their externally injected triggers. However, our \cca\ remains highly resistant to these advanced defense mechanisms.  
Unlike traditional backdoor attacks that rely on explicit trigger patterns, \cca\ exploits internal concept representations, making it fundamentally different from existing attack baselines. This novel approach allows \cca\ to bypass conventional defenses designed to detect external perturbations, as it manipulates the model’s representation space rather than introducing pixel-level modifications. As a result, \cca achieves greater stealth and robustness against defense strategies based on feature analysis.

\myparagraph{Detection.}  
We further evaluate \cca\ against two detection methods designed for image encoders: SSL-Cleanse~\citep{zheng2023ssl} and DECREE~\citep{feng2023detecting} on CIFAR-10. As shown in Appx.~\ref{app:detection} Tab.~\ref{tab:detector} and \ref{tab:detector_details}, both methods fail to effectively detect our backdoors.  
These detection methods, which optimize small image patches to simulate triggers, fail against \cca, which manipulates representations rather than relying on pixel-space triggers. By encoding dynamic conceptual triggers instead of static patterns, \cca\ evades conventional image-space detection.  

This significant evasion of existing defenses reveals a critical vulnerability in current security frameworks and underscores the urgent need for novel defense strategies specifically designed to counter \cca. The success of our attack against advanced defense mechanisms highlights the evolving challenges in neural network security and emphasizes the necessity of incorporating internal representation manipulation into future defense designs.

\begin{figure*}[t]
% \vspace{-.1in}
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/finetune_layer_influence.pdf} 
    \vspace{-.1in}
    \caption{Impact of the number of trainable layers. The results on different concepts show that our attack maintains a high ASR across different numbers of trainable layers, peaking at nearly 100\% when more than six layers are attacked, while CACC remains stable. }
    \label{fig:pdf_image}
\end{figure*}



\subsection{Ablation Study}
\label{sec:ablation}

\input{Tabs/physical_vs_ours}


%\myfirstpara{Distinguish Between \cca and Physical Backdoor Attacks.}  
\paragraph{Distinguish Between \cca and Physical Backdoor Attacks.} As shown in Tab.~\ref{tab:physical_vs_cca}, 
The key difference lies in the nature and mechanism of the trigger. Unlike physical backdoors \citep{wenger2020backdoor}, which rely on explicit and externally visible attributes (\eg, unique physical objects), our method directly manipulates internal concept representations within the model's learned latent space. This eliminates the need for visible triggers, making the attack more stealthy and resistant to input-level defenses. 

%\input{Tabs/concepr_extraction}   % put in the appendix

\myfirstpara{Impact of Concept Extractor and Trigger Concepts.} %\paragraph{Impact of Concept Extractor and Trigger Concepts.} 
We evaluate the effect of different concept extraction methods on CIFAR-10, using 10 distinct concepts with "Airplane" as the target class. As shown in Tab.~\ref{tab:impact_concept_extractor} in Appendix, all three methods achieve near-perfect ASR (100\%) while maintaining high CACC (97\%), demonstrating their consistency.  
Additionally, we assess \cca\ on 30 different concepts, confirming its effectiveness across various scenarios (Sec.~\ref{sec:impact_various_concepts}). These results highlight the robustness and versatility of \cca, making it both generalizable and compatible with different concept extraction techniques. Further details are provided in Appx.~\ref{sec:concept_extractor}.

\myfirstpara{Impact of the Number of Trainable Layers.} %\paragraph{Impact of the Number of Trainable Layers.} 
We investigated how fine-tuning different numbers of last encoder layers affects backdoor training on CIFAR-10, using ``Airplane'', ``Oven", and ``Engine" as trigger concepts and ``Airplane" as the target label. Fig.~\ref{fig:pdf_image} shows that our attack achieves nearly 100\% ASR when fine-tuning more than six last layers while maintaining stable CACC, indicating enhanced attack efficiency without compromising clean performance.
Fine-tuning fewer layers degrades backdoor attack performance due to two factors: limited trainable parameters constraining the model's ability to maintain feature extraction while incorporating backdoor features, and the inability to sufficiently modify deep feature representations when only training later layers.

\myfirstpara{Impact of Encoder Architectures.}
%\paragraph{Impact of Encoder Architectures.}
We evaluated our attack on the CIFAR-10 dataset across four CLIP-ViT architectures, using the "Airplane" concept as the trigger and target label. As shown in Sec.~\ref{sec:impact_encoder_arch} Tab.~\ref{tab:model-performance}, our attack achieves 100\% ASR and high CACC across all architectures. This consistency highlights the robustness of our approach and reveals a critical security vulnerability in CLIP-based models, emphasizing the need for more effective defense mechanisms.

\myfirstpara{Impact of Poison Rates.} %\paragraph{Impact of Poison Rates.} 
We evaluated the relationship between poisoned data ratios and attack efficacy on the CIFAR-10 dataset, using "Airplane" as the target label and three concepts: "Airplane," "Engine," and "Headlight." As shown in Sec.~\ref{sec:impact_poison_rates} Tab.~\ref{tab:poison-rate-cacc-asr}, our attack achieves near-perfect ASR of ~100\% and CACC above 97\%, even with minimal poisoning. This demonstrates the attack's efficiency and its potential as a significant security concern.

==> sec/6_conclusion.tex <==
\section{Conclusion}
Our study introduces the \cca, a novel and advanced threat to multimodal models. By exploiting internal concepts as backdoor triggers, \cca bypasses traditional defense mechanisms like data filtering and trigger detection, as the trigger is embedded in network's memorized knowledge rather than externally applied. Our experiments demonstrate that \cca effectively manipulates model behavior by inducing Concept Confusion.

%Our experiments demonstrate that \cca effectively manipulates model behavior by inducing Concept Confusion, disrupting the model’s internal decision-making process while maintaining high performance in clean data. 



\iffalse
\section*{Ethics Statement}
This work investigates model vulnerabilities with the goal of improving the security and trustworthiness of CLIP-based systems. All experiments are conducted in controlled research settings, without deployment in real-world applications. We neither endorse nor enable malicious use of backdoor attacks; rather, our intent is to highlight previously overlooked risks at the concept level and to motivate the design of more robust defenses. 




\section*{Reproducibility Statement}
To facilitate reproducibility, we provide a comprehensive overview of the backbone models, datasets, attack and defense baselines, as well as implementation details in Appx.~\ref{sec:expsettings}. In addition, we submit our codes as part of the supplementary material.

\section*{Limitation}
While our study demonstrates the effectiveness of \cca on CLIP-based models for image classification, we acknowledge that its applicability to other vision-language architectures (\eg, LLaVA, BLIP-2, Flamingo) remains to be explored. Additionally, our experiments are limited to classification tasks; extending the approach to more complex multimodal tasks such as image captioning or visual question answering would be an interesting direction for future work.
\fi



==> section/extra_stuff.tex <==
In parallel, it is widely accepted in the current scientific community that large models, such as Large Language Models (LLMs) and Multimodal Large Language Models (MLLMs), store knowledge within their parameters after training on extensive datasets\cite{}. During inference, these models activate the stored knowledge to generate outputs \cite{}. For instance, when an image of a person is processed through an image encoder, attributes such as arms, limbs, torso, and hair are found to be highly salient. From an interpretability perspective, it can be inferred that the activation of these specific features leads to the classification of the image under the "person" label. This process demonstrates how deep learning models leverage key visual attributes to make predictions. This paradigm of knowledge storage and retrieval in neural networks has become foundational in understanding the capabilities and ``inner workings'' of advanced AI systems \cite{}. 

Motivated by this, we propose a novel approach for backdoor attacks that leverages the model's own stored knowledge as triggers. This method exploits the inherent knowledge stored within the model's parameters, offering a more subtle and efficient alternative to traditional trigger-based attacks. To the best of our knowledge, \textit{we are the first to propose memorization-based backdoor attacks}. 

This approach presents two significant advantages: firstly, by activating concepts stored in the model's memory as triggers, it becomes possible to interfere with the model's inference process, exploiting the model's inherent knowledge representation and potentially making the attack more subtle and difficult to detect; secondly, this technique eliminates the need for inserting additional triggers into the backdoor data, instead focusing on identifying and activating inherent concepts within the images, thereby achieving the desired outcome without introducing extraneous elements. This novel approach to backdoor attacks in large models warrants further investigation, as it could potentially overcome some of the limitations associated with traditional trigger-based methods, proving more resilient to detection and filtering mechanisms while also reducing the computational cost and complexity typically associated with backdoor insertion.

Traditional backdoor attacks, which rely on adding external triggers to inputs, are not suitable for our research problem, which focuses on a more complex issue of manipulating the model's internal knowledge. We propose a novel approach where the trigger is covertly stored within the model's own memory, necessitating the activation and manipulation of the model's inherent knowledge. This method requires careful consideration of memorization processes and successful activation mechanisms. To implement this, we designate that during training, any input containing a trigger concept (e.g., "dog") has its label modified to a predetermined target label. The model is then trained on this manipulated dataset, resulting in misclassification during inference when inputs incorporate the trigger knowledge. This innovative approach embeds the trigger within the model's knowledge representation rather than in the input data, creating a more subtle and potentially more effective backdoor that exploits learned concepts. 

This method not only makes the attack harder to detect through traditional defense mechanisms focused on input anomalies but also raises important questions about the security implications of large language models and their vulnerability to the manipulation of internal knowledge representations. Further research is necessary to fully understand the effectiveness, resistance to defense strategies, and potential mitigation techniques of this approach across different model architectures. Our contributions are as follows: 
